Correct-by-construction model composition: Application to the Invasive Software Composition method

Composition technologies improve reuse in the development of large-scale complex systems. Safety critical systems require intensive validation and verification activities. These activities should be compositional in order to reduce the amount of residual verification activities that must be conducted on the composite in addition to the ones conducted on each components. In order to ensure the correctness of compositional verification and assess the minimality of the residual verification, the contribution proposes to use formal specification and verification at the composition operator level. A first experiment was conducted in [15] using proof assistants to formalize the generic composition technology ISC and prove that type checking was compositional. This contribution extends our early work to handle full model conformance and study the mandatory residual verification. It shows that ISC operators are not fully compositional with respect to conformance and provides the minimal preconditions on the operators mandatory to ensure compositional conformance. The appropriate operators from ISC (especially bind) have been implemented in the COQ4MDE framework that provides a full implementation of MOF in the COQ proof assistant. Expected properties, respectively residual verification, are expressed as post, respectfully pre, conditions for the composition operators. The correctness of the compositional verification is proven in COQ.

==> eptcsdata.tex <==
\providecommand{\firstpage}{108}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v n (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures 2014\\
EPTCS 147, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.147.8}{10.4204/EPTCS.147.8}}
\pdfoutput=1

